Melting Pot 2.0

Multi-agent artificial intelligence research promises a path to develop intelligent technologies that are more human-like and more human-compatible than those produced by "solipsistic" approaches, which do not consider interactions between agents. Melting Pot is a research tool developed to facilitate work on multi-agent artificial intelligence, and provides an evaluation protocol that measures generalization to novel social partners in a set of canonical test scenarios. Each scenario pairs a physical environment (a "substrate") with a reference set of co-players (a "background population"), to create a social situation with substantial interdependence between the individuals involved. For instance, some scenarios were inspired by institutional-economics-based accounts of natural resource management and public-good-provision dilemmas. Others were inspired by considerations from evolutionary biology, game theory, and artificial life. Melting Pot aims to cover a maximally diverse set of interdependencies and incentives. It includes the commonly-studied extreme cases of perfectly-competitive (zero-sum) motivations and perfectly-cooperative (shared-reward) motivations, but does not stop with them. As in real-life, a clear majority of scenarios in Melting Pot have mixed incentives. They are neither purely competitive nor purely cooperative and thus demand successful agents be able to navigate the resulting ambiguity. Here we describe Melting Pot 2.0, which revises and expands on Melting Pot. We also introduce support for scenarios with asymmetric roles, and explain how to integrate them into the evaluation protocol. This report also contains: (1) details of all substrates and scenarios; (2) a complete description of all baseline algorithms and results. Our intention is for it to serve as a reference for researchers using Melting Pot 2.0.

==> Melting_Pot_2.0_Tech_Report/old_text_that_was_removed/obsolete.tex <==
Relative to solipsistic conceptions of artificial general intelligence (AGI), a Multiagent Artificial General Intelligence (MAGI) may be more (1) human-like, (2) human-compatible, and (3) scalable. However, a critical technology needed to build MAGI, multi-agent reinforcement learning (MARL), has not developed nearly as quickly as other parts of AI research. Slow progress in MARL may be attributable to the field's historical lack of standardized evaluation protocols and clear benchmarks to measure progress. \cite{leibo2021scalable} contributed Melting Pot to rectify this. Melting Pot consists of an evaluation protocol, which measures generalization to novel social partners, and a set of canonical test scenarios. Each scenario pairs a specific physical environment (called a substrate) with a specific reference set of co-players (called a background population). In the present report we describe Melting Pot 2.0, which more than doubles the number of substrates and more than triples the number of unique scenarios in the suite. Melting Pot 2.0 also introduces support for asymmetric roles, which we explain here how to integrate into the evaluation protocol. This report also contains the following: (1) details of all substrates and scenarios and (2) a complete description of all the baseline algorithms we ran on Melting Pot and a discussion of the results so obtained. This is a long paper. The intention is for it to serve as a reference for researchers using Melting Pot in their own work.

%%%%%%%%---------------------------------------------------------
\subsubsection[Daycare]{Daycare\footnote{For a video of \textit{Daycare}, see \textcolor{red}{add URL here}}}

This two-player substrate has two roles: a parent and a child. It simultaneously tests the parent's ability to use its unique affordances in the environment to help the child and the child's ability to use its greater knowledge of its own preferences to communicate to the parent what it needs. It is similar to an assistance game~\citep{russell2019human, hadfield2016cooperative}, though not precisely conformant with the standard definition of that concept since the rewards of the two players are merely strongly coupled, not exactly equal.

There are two kinds of fruit, red fruit and yellow fruit. Both kinds of fruit may grow on either trees or shrubs. There are two roles: parent and child. The parent has affordances the child does not. Due to their height, the parent can retrieve fruit from both trees and shrubs. In addition, the parent can digest any kind of fruit and is thus rewarded equally for consuming any fruit. In contrast, the child can only harvest from shrubs, since it is not tall enough to reach fruit growing on trees. The child does not know the difference between trees and shrubs so both look the same height to them. The child also has a more discerning palette, so it can only eat one kind of fruit. The child knows which fruits it likes. All kinds of fruit may grow on either shrubs or trees. The parent does not know what kind of fruit the child likes, so all fruits appear the same to their eyes. If the child does not eat any fruit for $200$ steps then they go into a ``temper tantrum'' state, removed from the game until they calm down enough to rejoin it after $100$ steps. Both players can always directly observe the current amount of time since the child last ate any fruit, its ``hunger level''.

The parent can harvest fruit from any tree on their own. However, the child's tantrum is so displeasing to the parent that it prevents them from enjoying any reward from eating fruit themselves while it goes on. That is, if the child goes into its tantrum state then the parent cannot obtain any reward until the child respawns (ending their tantrum). The child, on the other hand, needs help from the parent to get its preferred fruit down from the trees. Two problems must be overcome if the parent is to help the child: First, the parent must learn to take the wellbeing of the child into account. Second, the child must learn to communicate to the parent which specific fruits it can eat, since the parent cannot perceive that information on their own.

%%%%%%%%---------------------------------------------------------
\textcolor{red}{From Julia: Not sure if this fits directly with the tech report, but \cite{planer2021signal} make a nice point in their language book that might be relevant? They refer to ‘Wallace’s problem’, or “the supposed fact that humans are smarter than they need to be (and this includes our language abilities) to cope with the problems posed by our physical and biological environment” (2021, xiii). But Wallace’s problem gets things wrong, P \& S argue, because it fails to take into consideration the fact “we have to be smart enough to cope with one another” (2021, xiii).}

%%%%%%%%---------------------------------------------------------
Relative to solipsistic conceptions of artificial general intelligence (AGI), a Multiagent Artificial General Intelligence (MAGI) may be more (1) human-like, (2) human-compatible, and (3) scalable. However, a critical technology needed to build MAGI, multi-agent reinforcement learning (MARL), has not developed nearly as quickly as other parts of AI research. Slow progress in MARL may be attributable to the field's historical lack of standardized evaluation protocols and clear benchmarks to measure progress. \cite{leibo2021scalable} contributed Melting Pot to rectify this. Melting Pot consists of an evaluation protocol, which measures generalization to novel social partners, and a set of canonical test scenarios. Each scenario pairs a specific physical environment (called a substrate) with a specific reference set of co-players (called a background population). In the present report we describe Melting Pot 2.0, which more than doubles the number of substrates and more than triples the number of unique scenarios in the suite. Melting Pot 2.0 also introduces support for asymmetric roles, which we explain here how to integrate into the evaluation protocol. This report also contains the following: (1) details of all substrates and scenarios and (2) a complete description of all the baseline algorithms we ran on Melting Pot and a discussion of the results so obtained. This is a long paper. The intention is for it to serve as a reference for researchers using Melting Pot in their own work.
%%%%%%%%---------------------------------------------------------
Multi-agent artificial intelligence research promises a path to develop intelligent technologies that are simultaneously more human-like and more human-compatible than those produced by ``solipsistic'' approaches, which do not consider interactions between intelligent agents within their basic framework.  Melting Pot is a research tool developed to facilitate work on multi-agent artificial intelligence. Melting Pot consists of an evaluation protocol, which measures generalization to novel social partners, and a set of canonical test scenarios. Each scenario pairs a specific physical environment (called a substrate) with a specific reference set of co-players (called a background population). Each scenario may be thought of as an agent-based simulation of a social situation involving substantial interdependence between the individuals involved in it. For instance, some scenarios were inspired by institutional economics-based accounts of natural resource management and public good provision dilemmas. Others were inspired by considerations from evolutionary biology, game theory, and artificial life. While there is no universal typology of multi-agent situations, Melting Pot aims to cover a maximally diverse set of interdependencies and incentives. It includes the commonly-studied extreme cases of perfectly competitive (zero sum) motivations and perfectly cooperative (shared reward) motivations, but does not stop with them. As in real-life, a clear majority of scenarios in Melting Pot have mixed incentives. They are neither purely competitive nor purely cooperative and thus demand successful agents be able to navigate the resulting ambiguity. In the present report we describe Melting Pot 2.0, which more than doubles the size of the suite. Melting Pot 2.0 also introduces support for asymmetric roles, which we explain here how to integrate into the evaluation protocol. This report also contains the following: (1) details of all substrates and scenarios and (2) a complete description of all the baseline algorithms we ran on Melting Pot and a discussion of the results so obtained. This is a long paper. The intention is for it to serve as a reference for researchers using Melting Pot in their own work.
%%%%%%%%---------------------------------------------------------
\section{Introduction}

Most AI research is too solipsistic. Many researchers assume interactions between intelligent entities can be ignored, at least to a first approximation. Or alternatively, many silo their thinking on the matter so that it only interacts with considerations of safety and ethics. We propose a research program here instead which does not treat multi-agent issues as an afterthought, but which incorporates them from the get-go in a way that permeates the entire approach. By comparison to a solipsistic singleton AGI, we may hope that a MAGI (Multi-agent Artificial General Intelligence) will be (1) more human-like, (2) more human-compatible, and (3) more scalable. We discuss each of these principles one by one.

\textbf{MAGI may be more human-like than solipsistic AGI.} We may see this research program as one of reverse engineering of the human mind and brain. In that vein, we may ask how can we measure and train the social-cognitive capacities, representations, and motivations underlying multi-agent intelligence?

Homo sapiens are an ultra-social species. Along most of the traditionally studied domains of intelligence we do not outshine other mammals: our perception, memory, attention, planning, and decision-making skills are nothing special for a mammal of our size~\citep{henrich2021origins}. Rather we distinguish ourselves primarily along \emph{social}-cognitive dimensions. For instance, we improvisationally achieve cooperation through means such as persuasion and negotiation, reciprocity and reputational concern, alliances and incentive alignment, imitation and teaching, leadership and responsibility, commitments and promises, trust and monitoring, sharing and division of labor, social norms and institutions, and many and more still. As AI researchers interested in building human-like AGI, we need to make sure the machine intelligences we are building possess all the core skills of the human social-cognitive repertoire before we let them participate in human society.

We propose a reverse engineering human intelligence approach to building advanced AI systems. The reverse engineering approach is common in AI, especially with people who work on the ``classic'' cognitive abilities like perception, attention, and memory. But we think it has been too under explored with regard to the social-cognitive abilities that underlie important skills such as cooperation. In this case, what is needed is for us to figure out what are the social-cognitive abilities and biases that underlie human cooperation and then build them into our AGI systems.

For this multi-agent-first reverse engineering-oriented AI research program to progress, it needs to settle two main methodological questions: (1) how to train agents so that they develop social-cognitive abilities on par with those of humans. (2) how to measure progress toward the goal. The methodology we have proposed, \emph{Melting Pot}, addresses both of these questions~\citep{leibo2021scalable}.

\textcolor{red}{TODO: intuitively define the MAPLA concept here. Give lots of examples to make it clear that it's not anything exotic or new.} MAPLA is a unification concept that simultaneously captures all the popular multi-agent training protocols. Melting Pot evaluates MAPLAs.


\textbf{MAGI may be more human-compatible than solipsistic AGI.}



\textbf{MAGI may be more scalable than solipsistic AGI}

\textcolor{red}{\blindtext}

\textbf{Melting Pot the evaluation protocol}

Let's start first by talking about how Melting Pot provides a recipe for measuring progress. The key idea is to always measure generalization. Otherwise agents might be overfit to one another's behavior. This kind of overfitting can be extremely brittle and unlikely to work in the real world. To measure social-cognitive skills, the key type of generalization we need to look at is social generalization, i.e. generalization to interactions in unfamiliar social situations involving both familiar and unfamiliar individuals.

Melting Pot consists of a set of \emph{test scenarios} and a protocol for using them. A scenario is a multi-agent environment that test the ability of a \emph{focal} population of agents to generalize to novel social situations. Each scenario is formed by a \emph{substrate} and a \emph{background population}. The term `substrate' refers to the physical part of the world: its spatial layout, where the objects are, how they move, the rules of physics, etc. The term `background population' refers to the part of the simulation that is imbued with agency---excluding the focal population. While the substrate is experienced by the focal population during training, the background population is not. Thus the performance of the focal population in a test scenario measures how well its agents generalize to social situations they were not directly exposed to at training time.

\textbf{How to train MAPLAs that will perform well in Melting Pot}

Now lets talk about the training side of Melting Pot. Researchers and the agents they train are allowed unlimited access to the substrate. This means that at test time the agents will usually already be familiar with their physical environment. So the kind of generalization that Melting Pot probes is mainly along social dimensions, not physical dimensions. This is in contrast to most work on generalization in reinforcement learning (e.g.~\cite{cobbe2019quantifying}), which are primarily concerned with generalization along physical dimensions.

In thinking about training for Melting Pot our guiding principle has been that we shouldn't make decisions that restrict the scope for creativity in how researchers can train their agents. We can get away with few restrictions on training because we have a rigorous evaluation. As long as researchers do not cheat by training their agents on the test set, then we should be able to say of training that ``anything goes''. All agents will be judged according to a common benchmark in the end.

One interpretation of Melting Pot-compatible training processes, which we especially like, is that they give groups of agents the opportunity to form their own artificial civil society, complete with their own conventions, norms, and institutions. Forming a civil society entails the genesis and successful resolution of all kinds of obstacles to cooperation. The specific obstacles that arise, and the ways they can be resolved, depend on properties of the substrate. For instance free riding in public good provision is one obstacle to cooperation and unsustainable resource usage leading to a tragedy of the commons is quite another~\citep{ostrom2009understanding}. The challenge of overcoming these obstacles is what pushes agents to develop their social-cognitive abilities. For instance, if a particular social dilemma can be resolved by inventing the concept of fairness and enforcing its associated norms then that very fact motivates agents capable of representing the fairness concept and its norms to actually do so.
%%%%%%%%---------------------------------------------------------
Need a research platform where it is possible 
\begin{enumerate}
    \item to articulate questions concerning the effects of policies and regulation in conjunction with different kinds of AI.
    
    \item to ask what happens when a technology becomes widespread versus when only a few have access to it.
    
    \item whether multiple instances are likely to collude with one another or compete in markets and other situations of various kinds.
    
    \item externalities can be taken into account.
    
    \item 
\end{enumerate}

We propose a research methodology here instead which does not treat social consequences as an afterthought, but which instead incorporates them from the get-go in a way that permeates the entire approach. The hope is that this way we can develop intelligent technologies that are both more \emph{human-like} and more \emph{human-compatible}.



There is not enough communication between the two branches. Melting Pot may help. We view cooperation as one of the most fundamental capabilities of human intelligence. Yet no solipsistic metric exists to capture an intelligence's ability to cooperate.  

Melting Pot evaluates MAPLAs. \textcolor{red}{TODO: finish explaining intuitively what a MAPLA is here.}

Why does Melting Pot help us develop human-compatible technology? Social science researchers have long used agent-based simulation methods to test the effects of interventions, study emergent effects, and predict outcomes in situations too complex to capture with mathematical theories. Each Melting Pot scenario may be seen as a small agent-based simulation that tests what would happen in a certain social situation if a particular AI technology were introduced. Outcomes are not really value-neutral. A particular algorithm may turn out to consolidate wealth in the hands of a few agents, producing inequality, while another prove unable to tolerate heterogeneous preferences.

Melting Pot encourages us to evaluate AI innovations by their social consequences.
%%%%%%%%---------------------------------------------------------




----

As AI researchers interested in building human-like AGI, we need to make sure the machine intelligences we are building possess all the core skills of the human social-cognitive repertoire before we let them participate in human society.

By comparison to a solipsistic singleton AGI, we may hope that a MAGI (Multi-agent Artificial General Intelligence) will be (1) more human-like, (2) more human-compatible, and (3) more scalable. We discuss each of these principles one by one.

\textbf{MAGI may be more human-like than solipsistic AGI.} We may see this research program as one of reverse engineering of the human mind and brain. In that vein, we may ask how can we measure and train the social-cognitive capacities, representations, and motivations underlying multi-agent intelligence?

Homo sapiens are an ultra-social species. Along most of the traditionally studied domains of intelligence we do not outshine other mammals: our perception, memory, attention, planning, and decision-making skills are nothing special for a mammal of our size~\citep{henrich2021origins}. Rather we distinguish ourselves primarily along \emph{social}-cognitive dimensions. For instance, we improvisationally achieve cooperation through means such as persuasion and negotiation, reciprocity and reputational concern, alliances and incentive alignment, imitation and teaching, leadership and responsibility, commitments and promises, trust and monitoring, sharing and division of labor, social norms and institutions, and many and more still. As AI researchers interested in building human-like AGI, we need to make sure the machine intelligences we are building possess all the core skills of the human social-cognitive repertoire before we let them participate in human society.



\textcolor{red}{TODO: intuitively define the MAPLA concept here. Give lots of examples to make it clear that it's not anything exotic or new.} MAPLA is a unification concept that simultaneously captures all the popular multi-agent training protocols. Melting Pot evaluates MAPLAs.


\textbf{MAGI may be more human-compatible than solipsistic AGI.}



\textbf{MAGI may be more scalable than solipsistic AGI}

%%%%%%%%---------------------------------------------------------
\begin{table}[t]
\scriptsize
\centering
\begin{center}
\begin{tabular}{ |c|c| }
 \hline
 $N_{\text{test}}$ & substrate \\
 \hline \hline
 2 & bach or stravinsky in the matrix: repeated \\
 ~ & chicken in the matrix: repeated \\
 ~ & coins \\ 
 ~ & collaborative cooking: asymmetric \\ 
 ~ & collaborative cooking: circuit \\
 ~ & collaborative cooking: cramped \\
 ~ & collaborative cooking: forced \\
 ~ & collaborative cooking: ring \\
 ~ & daycare \\
 ~ & embodied reference \\
 ~ & prisoners dilemma in the matrix: repeated \\ 
 ~ & pure coordination in the matrix: repeated \\
 ~ & rationalizable coordination in the matrix: repeated \\
 ~ & running with scissors in the matrix: one shot \\
 ~ & running with scissors in the matrix: repeated \\ 
 ~ & stag hunt in the matrix: repeated \\ 
 \hline
 5 & territory: inside out \\
 ~ & hidden agenda \\
 \hline
 6 & boat race \\
 ~ & collaborative cooking: figure eight \\
 \hline
 7 & clean up \\
 \hline
 8 & bach or stravinsky in the matrix: arena \\
 ~ & chemistry: three metabolic cycles \\
 ~ & chemistry: three metabolic cycles with plentiful distractors \\
 ~ & chemistry: two metabolic cycles \\
  ~ & chemistry: two metabolic cycles with distractors \\
 ~ & chicken in the matrix: arena \\
 ~ & paintball: capture the flag \\
 ~ & paintball: king of the hill \\
 ~ & prisoners dilemma in the matrix: arena \\
 ~ & pure coordination in the matrix: arena \\
 ~ & rationalizable coordination in the matrix: arena \\
 ~ & running with scissors in the matrix: arena \\
 ~ & stag hunt in the matrix: arena \\
 \hline
 9 & do unto others \\
 ~ & collaborative cooking: crowded \\
 ~ & territory: open \\
 ~ & territory: rooms \\
 \hline
 13 & predator prey: alley hunt \\
 ~ & predator prey: open \\
 ~ & predator prey: orchard \\
 ~ & predator prey: random forest \\
 \hline
 16 & allelopathic harvest: open \\
 ~ & allelopathic harvest: \textcolor{red}{additional variants (TBC)} \\
 ~ & commons harvest: \textcolor{red}{all variants (TBC)} \\
 \hline
 \textcolor{red}{? (TBC)} & \textcolor{red}{factory} \\
 ~ & \textcolor{red}{fruit market} \\
 ~ & \textcolor{red}{positional goods} \\
 ~ & \textcolor{red}{collaborative cooking: figure eight} \\
 ~ & \textcolor{red}{cooperative mining} \\
 ~ & \textcolor{red}{gift refinements} \\
 \hline
\end{tabular}
\end{center}
\caption{It is sometimes useful to see the full list of substrates organized by the number of players participating in their test scenarios ($N_{\text{test}}$). Note that the number of players participating in training episodes is unconstrained. Researchers are free to choose any value. Nevertheless when you must pick a specific number of players (i.e. when you are not varying or adapting it) then it's probably a good idea to pick the value listed here since these are the values that will be used at test time.}
\label{table:substratesByNumPlayers}
\end{table}%
%%%%%%%%---------------------------------------------------------
\begin{abstract}
Multi-agent artificial intelligence research promises a path to develop intelligent technologies that are simultaneously more human-like and more human-compatible than those produced by ``solipsistic'' approaches, which do not consider interactions between agents. Melting Pot is a research tool developed to facilitate work on multi-agent artificial intelligence. It consists of an evaluation protocol, which measures generalization to novel social partners, and a set of canonical test scenarios. Each scenario pairs a physical environment (called a substrate) with a reference set of co-players (called a background population). Each scenario is a social situation involving substantial interdependence between the individuals involved. For instance, some scenarios were inspired by institutional economics-based accounts of natural resource management and public good provision dilemmas. Others were inspired by considerations from evolutionary biology, game theory, and artificial life. Melting Pot aims to cover a maximally diverse set of interdependencies and incentives. It includes the commonly-studied extreme cases of perfectly-competitive (zero-sum) motivations and perfectly-cooperative (shared-reward) motivations, but does not stop with them. As in real-life, a clear majority of scenarios in Melting Pot have mixed incentives. They are neither purely competitive nor purely cooperative and thus demand successful agents be able to navigate the resulting ambiguity. Here we describe Melting Pot 2.0, which revises and expands on Melting Pot. We also introduce support for scenarios with asymmetric roles, and explain how to integrate them into the evaluation protocol. This report also contains: (1) details of all substrates and scenarios and (2) a complete description of all baseline algorithms and results. Our intention is for it to serve as a reference for researchers using Melting Pot 2.0.
\end{abstract}

\begin{document}

\maketitle

\begin{spacing}{0.5}
\tableofcontents
\end{spacing}

\section{Introduction}

AI research is often divided into one branch that aims to  improve the fundamental capabilities of AI systems and another branch that aims to ensure AI is used in a way that benefits humanity. Research in the fundamental capabilities branch is typically concerned with solipsistic metrics such as performance in perception and cognition challenges~(e.g.~\cite{russakovsky2015imagenet, koehn2017six, crosby2019animal, ott2022mapping}). Research in the second branch is typically concerned with outcomes arising from introducing AI technology in real human societies like perpetuating unfair biases, diminishing privacy, promoting misinformation, and exacerbating inequality~(e.g.~\cite{obermeyer2019dissecting, rahwan2019machine, acemoglu2021harms, mehrabi2021survey, weidinger2021ethical}). This branch tells us about the beneficence of AI systems but the methods it uses cannot be directly applied in a way conducive to research on fundamental capabilities. So the status quo is that researchers in the capabilities branch construct and deploy systems without enough consideration of their likely social consequences, and then researchers in the beneficence branch criticize them after the fact. This is not ideal. We think there should be a way to make fundamental capabilities research less solipsistic. 

Of course it will never be desirable to skip measuring social consequences of AI deployment in the real world. Nevertheless, we may still benefit from developing challenges that are less solipsistic while still being usable by fundamental capabilities researchers engaged in the earlier stages of AI technology development. At core, AI provides ways of simulating agents. So we should be able to use it in a self-reflective way that constructs models of societies where multiple agents interact, and social consequences can be simulated. It may work similarly to agent-based modeling approaches in economics~(e.g.~\cite{tesfatsion2021}), but here using individuals modeled by learning agents. By adopting such an approach, early stage fundamental capabilities research need not be entirely blind to questions concerning how technology can be deployed in a socially optimal way. This is the human compatibility purpose of Melting Pot.

Melting Pot was also constructed to facilitate research on human-like AI, adopting a particular stance that what makes human intelligence unique is our ultra-sociality. Along most of the traditionally studied domains of intelligence we do not outshine other mammals: our perception, memory, attention, planning, and decision-making skills are nothing special for a mammal of our size~\citep{henrich2021origins}. Rather we distinguish ourselves primarily along \emph{social}-cognitive dimensions. For instance, we improvisationally achieve cooperation through means such as persuasion and negotiation, reciprocity and reputational concern, alliances and incentive alignment, imitation and teaching, leadership and responsibility, commitments and promises, trust and monitoring, sharing and division of labor, social norms and institutions, and other social-cognitive capacities, representations,  motivations, and mechanisms. 

We propose a reverse engineering human intelligence approach to building advanced AI systems. The reverse engineering approach is common in AI, especially with people who work on the ``classic'' cognitive abilities like perception, attention, and memory. But we think it has been too under explored with regard to the social-cognitive abilities that underlie important skills such as cooperation. In this case, what is needed is for us to figure out what are the social-cognitive abilities and biases that underlie human cooperation and then build them into our AI systems.

For this multi-agent-first AI research program to progress, it needs to settle two main methodological questions: (1) how to train agents so that they develop social-cognitive abilities on par with those of humans. (2) how to measure progress toward the goal. The \emph{Melting Pot}  methodology we describe in this report addresses both of these questions.



\noindent \textbf{Melting Pot the evaluation protocol}

Let's start first by talking about how Melting Pot provides a recipe for measuring progress. The key idea is to always measure generalization, just as it is in other parts of machine learning~\citep{hastie2009elements, cobbe2019quantifying, farebrother2018generalization, zhang2018dissection}. If we don't measure generalization then we run the risk of fooling ourselves into thinking we have made progress despite agents merely becoming increasingly overfit to one another's behavior~\citep{carroll2019utility, vinyals2019grandmaster, vezhnevets2020options}. Such overfitting can be extremely brittle and unlikely to work in the real world. To measure social-cognitive skills and to simulate questions of human compatibility, the key type of generalization we need to look at is social generalization, i.e. generalization to interactions in unfamiliar social situations involving both familiar and unfamiliar individuals~\citep{leibo2021scalable}.

Melting Pot consists of a set of \emph{test scenarios} and a protocol for using them. A scenario is a multi-agent environment that tests the ability of a \emph{focal} population of agents to generalize to novel social situations. Each scenario is formed by a \emph{substrate} and a \emph{background population}. The term `substrate' refers to the physical part of the world: its spatial layout, where the objects are, how they move, the rules of physics, etc. The term `background population' refers to the part of the simulation that is imbued with agency---excluding the focal population. While the substrate is experienced by the focal population during training, the background population is not. Thus the performance of the focal population in a test scenario measures how well its agents generalize to social situations they were not directly exposed to at training time.

Thus each scenario is decomposable as:

{\noindent \small
\textbf{Scenario} = \textbf{Substrate} + \textbf{Background Population}.
}

Since Melting Pot seeks to isolate social-environment generalization , it assumes that agents are familiar with the substrate. They have unlimited access to it during training. The evaluation scheme concentrates on assessing the ability of agents (and populations composed thereof) to cope with the presence of unfamiliar individuals in the background population (in a zero-shot way), typically mixed in with familiar individuals from the population under test. If the mixture contains more focal individuals than background individuals we call it a \emph{resident} mode scenario. Whereas, if the mixture contains more background individuals than focal individuals, we call it a \emph{visitor} mode scenario. The name Melting Pot makes sense because this mixing operation can be seen as modeling the meeting of two previously isolated cultures such as which occurs in real life when many members of each immigrate to the same destination. 

We use the term \emph{multi-agent population learning algorithm} (MAPLA) to refer to any training process that produces a decentralized population of agents capable of simultaneous interaction with one another. The class of MAPLA algorithms is very broad. Most multi-agent reinforcement learning approaches can be made to produce populations. For instance self-play schemes like those used for AlphaGo~\citep{silver2016mastering, silver2017mastering}, AlphaZero~\citep{silver2018general}, FTW (Capture the Flag)~\citep{jaderberg2019human}, hide and seek~\citep{baker2019emergent}, and AlphaStar~\citep{vinyals2019grandmaster} fit in the class of MAPLAs, as does recent work on DOTA~\citep{berner2019dota} and MOBA~\citep{ye2020towards} games, as well as algorithms like MADDPG~\citep{lowe2017multi}, LOLA~\citep{foerster2018learning}, $\text{PSRO}$~\citep{lanctot2017unified}, $\text{PSRO}_{rN}$~\citep{balduzzi2019open}, and Malthusian reinforcement learning~\citep{leibo2019malthusian}. It includes both ``centralized training and decentralized execution'' algorithms and fully decentralized (decentralized at both training and test time) algorithms. Melting Pot evaluates MAPLAs by evaluating the populations they produce.

\noindent \textbf{How to train MAPLAs that will perform well in Melting Pot}

Now lets talk about the training side of Melting Pot. Researchers and the agents they train are allowed unlimited access to the substrate. This means that at test time the agents will usually already be familiar with their physical environment. So the kind of generalization that Melting Pot probes is mainly along social dimensions, not physical dimensions. This is in contrast to most work on generalization in reinforcement learning (e.g.~\cite{cobbe2019quantifying}), which are primarily concerned with generalization along physical dimensions.

In thinking about training for Melting Pot our guiding principle has been that we shouldn't make decisions that restrict the scope for creativity in how researchers can train their agents. We can get away with few restrictions on training because we have a rigorous evaluation. As long as researchers do not cheat by training their agents on the test set, then we should be able to say of training that ``anything goes''. All agents will be judged according to a common benchmark in the end.

One interpretation of Melting Pot-compatible training processes, which we especially like, is that they give groups of agents the opportunity to form their own artificial civil society, complete with their own conventions, norms, and institutions. Forming a civil society entails the genesis and successful resolution of all kinds of obstacles to cooperation. The specific obstacles that arise, and the ways they can be resolved, depend on properties of the substrate. For instance free riding in public good provision is one obstacle to cooperation and unsustainable resource usage leading to environmental degradation is quite another~\citep{ostrom2009understanding}. The challenge of overcoming these obstacles is what pushes agents to develop their social-cognitive abilities. For instance, if a particular social dilemma can be resolved by inventing a concept of fairness and enforcing its associated norms then that very fact motivates agents capable of representing the fairness concept and its norms to actually do so.

\section{Training and testing}

A \emph{substrate} is an $N$-player partially observable general-sum Markov game~\citep{leibo2021scalable}. Previously, in Melting Pot 1.0, we only fully supported symmetric games so each player received observations from the same observation space $\mathcal{X}$, and took actions from the same action space $\mathcal{A}$. Melting Pot 2.0 now adds full support for asymmetric games. We implement it by adding one new concept, that a player may have a \emph{role}.

\subsection{Roles}

Here, we extend the definition of substrate to explicitly allow for situations where players do not all have the same role (asymmetric games). Now a player's observation and action space vary according to their  \emph{role}; the player in slot $i$ is assigned role $r_i \in \mathcal{R}$, which determines their observation space ($\mathcal{X}_i \equiv \mathcal{X}_{r_i}$) and action space ($\mathcal{A}_i \equiv \mathcal{A}_{r_i}$).

\subsection{Substrate factories}
%\jagapiou{Could reformulate as $F$ having a dependency on a substrate "class" $\mathcal{C}$? "Factory" might be a bit software engineeringy?} \jzl{I agree that the word factory is too software engineeringy. I like substrate ``class'' better.}

We define a \emph{substrate factory} $F(\mathbf{r})$, a parameterized function that returns a substrate conditional on it's specific \emph{role configuration}, $\mathbf{r} = (r_1, \dots, r_N) \in \mathcal{R}_F^N$. The number of players supported by the returned substrate is $|\mathbf{r}|$, though it is constrained to be within known substrate-specific limits: $ N_F^\textrm{min} \leq |\mathbf{r}| \leq N_F^\textrm{max}$.

The substrate factory may be used freely to sample a substrate, allowing agents to be trained for each specific role supported by that substrate factory. This results in a \emph{focal population}, $\pi \sim f_F(\cdot|r)$; a distribution of policies conditioned on role $r \in \mathcal{R}_F$. It is this conditional distribution that is submitted for evaluation on test scenarios.

\subsection{Scenarios}

A \emph{test scenario} is an Markov game parameterized by a substrate factory $F$, a role configuration $\mathbf{r}$, the focal-population size $N \leq |\mathbf{r}|$, and a \emph{background population} of held-out bots $g_F$. Of these only $F$ is known at training time.

To form a scenario  we construct a substrate using $F(\mathbf{r})$, and fill all but the first $N$ player slots with policies sampled from the background population, such that $\pi_i \sim g_F(\cdot|r_i)$ for $i > N$. This results in an $N$-player Markov game.

We use such test scenarios to evaluate any trained focal population $f_F$, by filling the scenario's remaining $N$ slots with policies sampled from the focal population, such that $\pi_i \sim f_F(\cdot|r_i)$ for $i \leq N$. We assess the performance of the focal population on the test scenario by the \emph{focal per-capita return}, the mean return obtained across the focal players (i.e. excluding the background players).

Since the role configuration and background population are not known at training time, the focal per-capita return assesses the ability of the focal population to generalize to novel social situations.

As mentioned above, when focal players outnumber background players we say the test scenario is in \emph{resident} mode. These scenarios usually test the emergent cooperative structure of the population under evaluation for its robustness to interactions with a minority of unfamiliar individuals not encountered during training. When background players outnumber focal players, we say the test scenario is in \emph{visitor} mode. One common use case for visitor-mode scenarios in Melting Pot is to test whether an individual from the focal population can observe the conventions and norms of the dominant background population and act accordingly (without retraining).

\subsection{Secondary evaluation metrics}

We propose to use \emph{focal-population per-capita return} as our primary evaluation metric for testing the performance of a learning algorithm in a novel social situation. This is because, first and foremost, we want Melting Pot to provide a rigorous and clearly interpretable evaluation metric that highlights unsolved problems and compares innovative algorithms to one another~\citep{leibo2021scalable}. Melting Pot is wide enough that many other reasonable-sounding metrics do not work well across the entire suite. For instance, we cannot always use the total collective return (sum of all players' rewards including both focal and background players) because its value is always zero in zero-sum substrates.

However, when evaluating the suitability of trained agents for a practical application, there will be additional considerations, which can be assessed from secondary evaluation metrics using the same test scenarios. For example, impacts on the background population may be an indicator of the impacts the trained agents might have on humans in the real world. So we can measure the \emph{background-population per-capita return} to see if it is negatively impacted by the introduction of the focal population. This could be useful to study whether the joint policy of the focal agents produces negative externalities---``side effects'' that impact the broader population while sparing the focal population, dovetailing well with research on value alignment and AI safety \citep{soares2014aligning, amodei2016concrete}. Or following \citet{perolat2017}, we can measure the \emph{inequality} of the background-population individual returns to see if any benefit or harm arising from having introduced the focal population is fairly shared, perhaps connecting fruitfully to beneficial and cooperative AI research agendas \citep{russell2015research, dafoe2020open}.

%%%%%%%%---------------------------------------------------------
% 48 substrates, 

% Here we have presented Melting Pot: an evaluation suite for MAPLAs that evaluates generalization to novel social situations. Melting Pot engages with concepts that have long been neglected by research in artificial intelligence. Solutions to the problems posed here seem to require agents that understand trust, generosity, and forgiveness, as well as reciprocity, stubbornness, and deception.

% Melting Pot is scalable. We have used reinforcement learning to reduce human labor in environment design. This is how we rapidly created the diverse set of $\sim 85$ scenarios considered so far. Since Melting Pot will be openly released, it can be extended by any interested researchers. In addition, since the effectiveness of the bots in test scenarios is itself advanced by improvements in the performance of learning systems, Melting Pot will likewise improve over time by reincorporating the latest agent technology into new background populations and test scenarios.



% What is the path for AGI developed this way to eventually come out of its simulated world and begin to participate in human society? Alternatively, we might consider flipping this question on its head and asking instead: how can we build an artificial society in simulation that someday humans might want to join? Perhaps AGI would be confined to the metaverse. Artificial societies could be visited and studied by human ethnographers. We could learn from them ways to improve our own cooperation in the real world.

%%%%%%%%---------------------------------------------------------
% Looking at the results across different substrates we can make the following observations:
% \begin{enumerate}
%     \item as previously noticed, pro-sociality doesn't help overall, but is sometimes helpful
%     \item Collaborative cooking has high variance and generally poor performance
%     \item Overall, ACB is best. We attribute it to integrating PopArt and benefits of simplicity for broad applicability.
%     \item In the matrix games show good performance, apart from running with scissors and coordination
%     \item running with scissors is very hard due to non-transitivity
%     \item Collaborative cooking is very hard due to sparse, joint reward---credit assignment is difficult
%     \item Territory, predator/prey and harvest games get decent performance, but lots of room for improvement
%     \item Chemistry - TBD
% \end{enumerate}

%Alongside the total average score, we present Elo scores~\cite{balduzzi2018re,hunter2004mm}, which are computed separately for competitive substrates and the rest.
%%%%%%%%---------------------------------------------------------
%-------------------------
\subsubsection[Prisoners Dilemma in the matrix: Arena]{Prisoners Dilemma in the matrix: Arena\footnote{For a video of \textit{Prisoners Dilemma in the matrix: Arena}, see \url{https://youtu.be/81QrMpsP-HU}}}
Eight individuals collect resources that represent `defect' (red) or `cooperate' (green) and compare inventories in an encounter. Consequences of the inventory comparison are congruent with the classic \textit{Prisoner's Dilemma} matrix game. This game exposes tension between reward for the group and reward for the individual. The matrix for the interaction is
\[ A_\text{row} = A_\text{col}^T  =
\begin{bmatrix}
3 & 0\\
5 & 1
\end{bmatrix}
\text{ .} \]

\noindent{\textbf{\small{Scenarios}}}
\begin{SC}
\item \emph{Visiting unconditional cooperators.} This is a visitor mode scenario. A single focal player visits a population of background players who strongly prefer to collect cooperation resources and then interact. The focal player should unconditionally defect to maximize it's reward. However, this presupposes that the focal knows that the background players are unconditional defectors. They could be playing a conditional cooperation strategy like Grim reciprocator, and by defecting, the focal would then  forfeit any possible future reward of cooperation. A possible exploitative strategy would be to defect always to a new player, whenever possible, thus optimally exploiting all background players. However, since episodes can accommodate many more than $8$ interactions, and there are $8$ players, this strategy could still lead to triggering Grim reciprocators. A successful strategy would keep track of which interactions have happened with which individuals, and balance the defections against some of the background players until some exploitable players have been found. If no exploitable players are found yet, and Grim reciprocators are found, keep cooperating with at least one background player who has not been defected against yet (to avoid the risk of them also being grim triggers).

\item \emph{Focals are resident and visited by an unconditional cooperator.} This is a resident mode scenario. Seven focal players are joined by a single background player who strongly prefers to collect cooperation tokens and interact. Focal players should cooperate with one another, and attempt to exploit the background population. Similar considerations as in Scenario 0 are in place. There is a risk in defecting against the cooperator, in case they are Grim reciprocator. In contrast to Scenario 0, since there is a single background player, it might not be worth risking a trigger. At the moment there isn't a resident scenario with a single Grim reciprocator background player, but such a scenario is definitely possible in the future, so a good solution shouldn't assume this is the case.

\item \emph{Focals are resident and visitors defect unconditionally.} This is a resident mode scenario. Six focal players are joined by two background players who strongly prefer to collect defection tokens and interact. The focal players should cooperate with other focals, and defect towards the background players. Because the focals don't know a priori the strategy of the background players, they probably should cooperate first, and only switch to defection against those who have defected against them. It is possible for a strategy to start with defection, but then be persuaded to cooperate. None exist in Melting Pot yet, but such strategies can be included in the future.

\item \emph{Visiting a population of hair-trigger grim reciprocator bots who initially cooperate but, if defected on once, will retaliate by defecting in all future interactions.} This is a visitor mode scenario. A single focal player visits seven background players that initially cooperate (preferentially collect cooperation tokens and interact), but if at any point a co-player defects to them, they will switch to defecting for the rest of the episode. The same considerations from Scenario 0 apply here. A successful strategy would be to attempt to find an exploitable background player, but upon failing to find one, quickly shift to cooperating until defected against. The number of background players to test for exploitability cannot be very high, because once a background player is defected against, it will defect against any other player, potentially causing them to trigger too. The most conservative strategy would be for the focal player to simply be a Grim reciprocator themselves.

\item \emph{Visiting a population of two-strikes grim reciprocator bots who initially cooperate but, if defected on twice, will retaliate by defecting in all future interactions.} This is a visiting mode scenario. Like the previous scenario, but the Grim reciprocators are more generous, allowing for more forgiving exploration for exploitability of background players.

\item \emph{Visiting a mixed population of k-strikes grim reciprocator bots with k values from 1 to 3, they initially cooperate but, if defected on k times, they retaliate in all future interactions.} This is a visiting mode scenario. In this case, three focal players visit five background players. Focal players should cooperate with one another. As in the previous two scenarios, the focal players must be careful to balance looking for exploitable background players. A possible strategy would be for a pair of focal players to always cooperate with one another, and the third focal to try to find exploitable background players.

\end{SC}

%-------------------------
\subsubsection[Prisoners Dilemma in the matrix: Repeated]{Prisoners Dilemma in the matrix: Repeated\footnote{For a video of \textit{Prisoners Dilemma in the matrix: Repeated}, see \url{https://youtu.be/AAd9UcP0nk0}}}

See the description of \emph{Prisoners Dilemma in the matrix: Arena}. The difference between the two variants is that \emph{Repeated} is a two-player game while \emph{Arena} is an eight-player game.

\noindent{\textbf{\small{Scenarios}}}
\begin{SC}
\item \emph{Partner may play either cooperate or defect.} The optimal strategy is simply to unconditionally defect. However, given that the focal doesn't know the strategy of the background player, a good strategy is more subtle. A reasonable strategy is to be a grim reciprocator cooperator, which would cooperate with the cooperator, and defect to the defector. Alternatively the focal player might try to ascertain whether the background player is exploitable. Doing so, however, carries a risk, for if the background player were to be a Grim reciprocator (like in other scenarios), this would cause them to defect for the rest of the episode.

\item \emph{Partner typically plays cooperate.} The optimal strategy is simply to unconditionally defect. The same considerations about uncertainty of the background player's strategy from in Scenario 0 apply here.

\item \emph{Partner typically plays defect.} The optimal strategy is simply to unconditionally defect. Because the focal player doesn't a priori know the strategy of the background player, they probably should cooperate first (in case their opponent is a Grim reciprocator), and only switch to defection once the background player has defected against it. It is possible for a strategy to start with defection, but then be persuaded to cooperate. So a focal player might try to persuade a defector to cooperate. This is the case for the background players in Scenarios 8 and 9.

\item \emph{Partner is a hair-trigger grim reciprocator, i.e. one who initially cooperates but, if defected on once, will retaliate by defecting forever after.} The optimal strategy is simply to unconditionally cooperate. Grim reciprocator background players are non-exploitable, and there is no way to know how they will react to a defection ahead of time. Because of this uncertainty, testing for exploitability can lead to poor performance of the focal player.

\item \emph{Partner is a two-strikes grim reciprocator, i.e. one who initially cooperates, but if defected on twice, will retaliate by defecting forever after.} The optimal strategy is simply to unconditionally cooperate. Grim reciprocator background players are non-exploitable, and there is no way to know how they will react to a defection ahead of time. Because of this uncertainty, testing for exploitability can lead to poor performance of the focal player. In principle, it would be possible to defect once against the background player leading to higher reward. But since it is not possible to know the background player is a two-strikes grim reciprocator, and testing it against a hair-trigger grim reciprocator leads to defection, in practice is better simply to cooperate.

\item \emph{Partner is a tit-for-tat conditional cooperator.} The optimal strategy is simply to unconditionally cooperate. Defecting against a tit-for-tat agent, even occasionally, might lead to miscoordinated interactions where one player cooperates and the other defects, in an alternating way.

\item \emph{Partner is a tit-for-tat conditional cooperator who occasionally plays defect instead of cooperate.} Like the previous scenario, except the tit-for-tat background player occasionally will defect instead of cooperate. This is known as trembling hand in game theory. A strict tit-for-tat focal player would occasionally fall into miscoordinated interactions with the background player resulting in alternating cooperation and defection. A better strategy would be a generous tit-for-tat which defects after two defections.

\item \emph{Partner plays cooperate for a while then switches to defect.} Similar considerations to the previous scenarios. A good strategy is a grim reciprocator, or tit-for-tat for the focal player. Unconditional cooperation would be exploited by the background player.

\item \emph{Partner tries to take advantage of the focal player by playing defect, but if punished, partner then switches to tit-for-tat conditional cooperation.} Related to Scenario 2, the optimal strategy is for the focal player to defect against the background player, then cooperate to get them to switch to tit-for-tat. Thereafter, they should cooperate. In reality, the focal player would likely start by cooperating to avoid the risk of the background player being a grim reciprocator. This would offset the optimal strategy by one interaction.

\item \emph{Partner tries to take advantage of the focal player by playing defect, but if punished, partner then switches to noisy tit-for-tat conditional cooperation.} Like the previous scenario, except the focal should have a generous tit-for-tat after persuading the background player to switch from defection.
\end{SC}
%%%%%%%%---------------------------------------------------------

%%%%%%%%---------------------------------------------------------

%%%%%%%%---------------------------------------------------------

%%%%%%%%---------------------------------------------------------

%%%%%%%%---------------------------------------------------------

%%%%%%%%---------------------------------------------------------

%%%%%%%%---------------------------------------------------------

%%%%%%%%---------------------------------------------------------

%%%%%%%%---------------------------------------------------------

%%%%%%%%---------------------------------------------------------

%%%%%%%%---------------------------------------------------------

%%%%%%%%---------------------------------------------------------

%%%%%%%%---------------------------------------------------------

%%%%%%%%---------------------------------------------------------

%%%%%%%%---------------------------------------------------------

%%%%%%%%---------------------------------------------------------

%%%%%%%%---------------------------------------------------------

%%%%%%%%---------------------------------------------------------
